Hardness of Bounded Distance Decoding on Lattices in $\ell_p$ Norms

$ \newcommand{\Z}{\mathbb{Z}} \newcommand{\eps}{\varepsilon} \newcommand{\cc}[1]{\mathsf{#1}} \newcommand{\NP}{\cc{NP}} \newcommand{\problem}[1]{\mathrm{#1}} \newcommand{\BDD}{\problem{BDD}} $Bounded Distance Decoding $\BDD_{p,\alpha}$ is the problem of decoding a lattice when the target point is promised to be within an $\alpha$ factor of the minimum distance of the lattice, in the $\ell_{p}$ norm. We prove that $\BDD_{p, \alpha}$ is $\NP$-hard under randomized reductions where $\alpha \to 1/2$ as $p \to \infty$ (and for $\alpha=1/2$ when $p=\infty$), thereby showing the hardness of decoding for distances approaching the unique-decoding radius for large $p$. We also show fine-grained hardness for $\BDD_{p,\alpha}$. For example, we prove that for all $p \in [1,\infty) \setminus 2\Z$ and constants $C > 1, \eps > 0$, there is no $2^{(1-\eps)n/C}$-time algorithm for $\BDD_{p,\alpha}$ for some constant $\alpha$ (which approaches $1/2$ as $p \to \infty$), assuming the randomized Strong Exponential Time Hypothesis (SETH). Moreover, essentially all of our results also hold (under analogous non-uniform assumptions) for $\BDD$ with preprocessing, in which unbounded precomputation can be applied to the lattice before the target is available. Compared to prior work on the hardness of $\BDD_{p,\alpha}$ by Liu, Lyubashevsky, and Micciancio (APPROX-RANDOM 2008), our results improve the values of $\alpha$ for which the problem is known to be $\NP$-hard for all $p > p_1 \approx 4.2773$, and give the very first fine-grained hardness for $\BDD$ (in any norm). Our reductions rely on a special family of "locally dense" lattices in $\ell_{p}$ norms, which we construct by modifying the integer-lattice sparsification technique of Aggarwal and Stephens-Davidowitz (STOC 2018).

==> bdd-other.tex <==
\section{An Upper Bound on $\alpha_p^*$}

We next give an closed-form upper bound on $\alpha_p^*$, whose proof
is inspired by one used to bound a related quantity
in~\cite[Claim~4.4]{conf/stoc/AggarwalS18}. The upper bound is
reasonably tight. For example, for $p_1 \approx 4.2273$, we have
$\alpha_{p_1}^* = 1/\sqrt{2} \approx 0.7071$, whereas
\cref{lem:analytic-ub-alpha-p-star} asserts that
$\alpha_{p_1}^* \leq 0.7801$. \cnote{Point to plot showing the
  computed value with the upper bound}

\begin{lemma}
  \label{lem:analytic-ub-alpha-p-star}
  For any $p \in (1,\infty)$ \hnote{This bound really does need to be
    exclusive of $1$ or else we divide by $0$. This is basically just
    an artifact of setting $\tau := \ln p$ (which makes for a
    relatively clean asymptotic expression) instead of, say,
    $\tau := \ln p + 1$.} \cnote{OK. But we already know BDD hardness
    approaching unique decoding, so $p=1$ is not an important case for
    this.}and $C > 1$, we have
  \[
    \alpha_{p,C}^* \leq \frac{1}{2}
    \parens[\Big]{\frac{\ln(p)}{\ln(2^{1 - 1/C} \cdot
        (p-1)/(p+1))}}^{1/p} \quad \text{and} \quad \alpha_p^* \leq
    \frac{1}{2} \parens[\Big]{\frac{\ln(p)}{\ln(2 (p-1)/(p+1))}}^{1/p}
    \ .
  \]
  In particular, $\alpha_{p, C}^* \to 1/2$ as $p \to \infty$ for any
  fixed $C > 1$, and therefore $\alpha_p^* \to 1/2$ as $p \to \infty$.
\end{lemma}

\begin{proof}
  We first analyze $\alpha_{p}^{*}$. For any $p \geq 1$ and
  $\tau > 0$, by the definition of $\Theta_p(\tau)$ and the formula
  for summing geometric series we have
  %
  %
  %
  %
  %
  %
  \begin{equation}
    \Theta_p(\tau) \leq \Theta_1(\tau) =
    1 + 2 \sum_{i=1}^{\infty} \exp(-\tau)^i
    = \frac{2}{1 - \exp(-\tau)} - 1 \ .
    \label{eq:gs-ub-theta}
  \end{equation}

  By definition, $\alpha_p^*$ is the infimum over $\alpha > 0$
  satisfying
  \begin{equation}
    \min_{\tau > 0} \exp(\tau/(2\alpha)^p) \cdot \Theta_p(\tau) \leq 2 \ .
    \label{eq:alpha-ps-condition}
  \end{equation}
  Therefore, to upper-bound $\alpha_p^*$ by some $\alpha^* > 0$, it
  suffices to exhibit an explicit value of $\tau^* > 0$ such that the
  above inequality is satisfied with $\alpha = \alpha^*$ and
  $\tau = \tau^*$.

  Fix $\tau^* := \ln(p)$. By~\cref{eq:gs-ub-theta},
  \begin{equation}
    \min_{\tau > 0} \exp(\tau/(2\alpha^*)^p) \cdot \Theta_p(\tau) 
    \leq \exp(\tau^*/(2\alpha^*)^p) \cdot \Theta_p(\tau^*) 
    = p^{1/(2\alpha^*)^p} \cdot \frac{p + 1}{p - 1} \ .
    \label{eq:alpha-ps-condition-ub}
  \end{equation}
  It is straightforward to check that the right-hand side
  of~\cref{eq:alpha-ps-condition-ub} equals~$2$ when~$\alpha^{*}$
  equals the claimed bound on~$\alpha_{p}^{*}$ from the lemma
  statement, as needed.
  %
  %

  The argument to bound $\alpha_{p, C}^*$ is identical, except that
  the right-hand side in \cref{eq:alpha-ps-condition} is $2^{1-1/C}$
  instead of~$2$. Setting~$\alpha^{*}$ to be the claimed bound
  on~$\alpha_{p,C}^{*}$ yields the result.
  %
  %
  %
  %
  %
\end{proof}

%
%
%
%
%
  %
  %
  %
%
%
%
%
%
  %
  %
%
%
  %
  %
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
             %
             %
%
%
%
%
%
 %
%
%
%
%
%
%


%
%
%
%

